Critical ride comfort detection for automated vehicles

In a future connected vehicle environment, an optimized route and motion planning should not only fulfill efficiency and safety constraints but also minimize vehicle motions and oscillations, causing poor ride comfort perceived by passengers. This work provides a framework for a large-scale and cost-efficient evaluation to address AV's ride comfort and allow the comparison of different comfort assessment strategies. The proposed tool also gives insights to comfort data, allowing for the development of novel algorithms, guidelines, or motion planning systems incorporating passenger comfort. A vehicle-road simulation framework utilizable to assess the most common ride comfort determination strategies based on vehicle dynamics data is presented. The developed methodology encompasses a road surface model, a non-linear vehicle model optimization, and Monte Carlo simulations to allow for an accurate and cost-efficient generation of virtual chassis acceleration data. Ride comfort is determined by applying a commonly used threshold method and an analysis based on ISO 2631. The two methods are compared against comfort classifications based on empirical measurements of the International Roughness Index (IRI). A case study with three road sites in Austria demonstrates the framework's practical application with real data and achieves high-resolution ride comfort classifications. The results highlight that ISO 2631 comfort estimates are most similar to IRI classifications and that the thresholding procedure detects preventable situations but also over- or underestimates ride comfort. Hence, the work shows the potential risk of negative ride comfort of AVs using simple threshold values and stresses the importance of a robust comfort evaluation method for enhancing AVs' path and motion planning with maximal ride comfort.

==> literature_review_temps.tex <==
PT studies: 
\begin{itemize}
    \item PHD thesis Förstberg 2000~\cite{ref:foerstberg} : Ride comfort and motion sickness in tilting trains
    \item Exploits the human response to different motions in public transportation, specifically trains
    \item Experiments provide empirical data (vehicle dynamics and answers to a questionnaire); regression analysis are then performed that identify that the most critical variables are motion does from the lateral and roll acceleration in the horizontal plane. 
    \item Due to the high low frequency content of vehicle dynamic signals, a model of provocation of motion sickness is proposed, showing that motion sickness has a time decay or leakage. 
\end{itemize}

\begin{itemize}
    \item Nguyen 2019: Insight into the lateral ride discomfort thresholds of young-adult bus passengers at multiple postures: Case of Singapore~\cite{ref:NGUYEN}
    \item Again studies the bus comfort by considering objective and subjective data
    \item Provides a nice table with different evaluation strategies and the inputs and parameters needed
    \item Linear regression model is fit to explain the correlation between the subjective ratings and the lateral acceleration and duration of a turning movement. 
    \item To model quality is modest and hence derived thresholds should be further investigated. 
\end{itemize}

\begin{itemize}
    \item Zhang 2014: Evaluating bus transit performance of Chinese cities: Developing an overall bus comfort model~\cite{ref:ZHANG}
    \item proposes a bus comfort model that is derived from subjective questionnaire results (take onboard of a city bus during the same trips) and physical parameters (such as noise, thermal comfort, vibration and acceleration. 
    \item a multiple linear regression model is fitted. 
\end{itemize}

\begin{itemize}
    \item Eboli 2016: Measuring bus comfort levels by using acceleration instantaneous values
    \item Again kinematic parameters are collected with a smartphone app and subjective data is collected with a questionnaire. 
    \item Out of the empirical analysis thresholds of comfort level. 
\end{itemize}


\begin{itemize}
    \item Castellanos 2014: Embedded system to evaluate the passenger comfort in public transportation based on dynamical vehicle behavior with user’s feedback
    \item An embedded system to localize discomfort in public transportation networks
    \item Identify the comfort results, a comfort index measurement (here the ISO2631) and a jerk threshold detection are utilized
    \item the results are simply based on a threshold detection algorithm. 
\end{itemize}

\begin{itemize}
    \item Förstberg 2003~\cite{ref:foerstberg2}: UIC comfort tests. Investigation of ride comfort and comfort disturbance on transition and circular curves
    \item Because of the general definition of the ISO2631, the UIC working group agreed on a UIC evaluation standard for trains. Nevertheless, the method used for defining the UIC standard is only valid for straight sections.
    \item Work investigates into the application and potential extension of the UIC standard on transition and circular curves.
    \item Study tries to find a correlation between passenger votes and UIC parameters (estimated with empirical data) but results do not show a clear picture. Bad correlations, low number of samples. 
\end{itemize}

IRI studies: 

\begin{itemize}
    \item Mucka et al 2020: International Roughness Index
     Thresholds Based on Whole-Body Vibration in Passenger Cars
     \item Estimation of the relationship between seat acceleration response and comfort reactions to ISO and IRI
     \item IRI thresholds proposed as a function of vehicle speed and road category. 
     \item Study contains measurements of nine different cars in six categories and a TTD of 1.8km. 
\end{itemize}


\begin{itemize}
    \item Elbanhawi 2015: In the passenger seat: Investigating ride comfort measures in autonomous cars~\cite{ref:elbanhawi}
    \item Review article of sate-of-the-art comfort assessments also in the context of path-planning algorithms for AVs
    \item Study underlines that their is a research gap and more research will be generated
\end{itemize}

AV focused studies: 
\begin{itemize}
    \item Eriksson 2015: Tuning for Ride Quality in
Autonomous Vehicle~\cite{ref:eriksson}
    \item lateral path planning algorithm
    \item based on a finite horizon linear quadratic controller
    \item studies shows differences in ride comfort when comparing
    normal and automated driving. 
    \item tuning the controller towards a better comfort for automated driving showed little to no improvement. 
\end{itemize}

\begin{itemize}
    \item Sun 2018: An Optimal Driving Strategy for the Ride Comfort Performance of
Intelligent Vehicles on Uneven Roads~\cite{ref:sun2018}
    \item Study works with an 7-DOF vehicle model and the ISO2631 to solve a Parto optimization problem
    \item An optimal driving strategy is derived by considering the comfort  (ISO2631) and driving requirements 
\end{itemize}

\begin{itemize}
    \item Salter 2019: Motion sickness in automated vehicles with forward and rearward facing seating orientations~\cite{ref:salter}
    \item The work considers the seat positioning (forward and rearward sitting)
    \item Study finds that with forward sitting a low risk of  motion sickness was reported but an increase of mean level of sickness with rearward sitting was reported, especially in urban driving conditions. 
    \item Study underlines the importance of testing different seating positions, speed profiles, etc.
\end{itemize}

%IRI

\textcolor{red}{Here we present the technical concept of the IRI and also discuss further the following topics}
\begin{itemize}
    \item \textcolor{red}{How is the data aquired specifially at AIT?}
    \item \textcolor{red}{How can IRI be linked to ride comort? Here we should find solid
    literature sources that support the utilized methodological concept. }
\end{itemize}
